A scalable architecture for distributed receive beamforming: analysis and experimental demonstration

We propose, analyze and demonstrate an architecture for scalable cooperative reception. In a cluster of N + 1 receive nodes, one node is designated as the final receiver, and the N other nodes act as amplify-and-forward relays which adapt their phases such that the relayed signals add up constructively at the designated receiver. This yields received SNR scaling linearly with N, while avoiding the linear increase in overhead incurred by a direct approach in which received signals are separately quantized and transmitted for centralized processing. By transforming the task of long-distance distributed receive beamforming into one of local distributed transmit beamforming, we can leverage a scalable one-bit feedback algorithm for phase synchronization. We show that time division between the long-distance and local links eliminates the need for explicit frequency synchronization. We provide an analytical framework, whose results closely match Monte Carlo simulations, to evaluate the impact of phase noise due to relaying delay on the performance of the one-bit feedback algorithm. Experimental results from our prototype implementation on software-defined radios demonstrate the expected gains in received signal strength despite significant oscillator drift, and are consistent with results from our analytical framework.

==> freq_synch_0824_AI.tex <==
\section{Frequency synchronization}
\label{sec:freq_synch}

\subsection{Implicit frequency synchronization}
\label{subsec:impl_freq_synch}

One major advantage of using a amplify-and-forward architecture for D-Rx beamforming is that, in principle, no frequency synchronization is required. Instead, it is possible to achieve \textit{implicit} frequency synchronization. To see this, suppose that the LO frequency offset between the transmitter and final receiver is denoted by $f_0$, and that the offset between the transmitter and the $i$-th relay is given by $f_{i1}$. The LO frequency offset between the $i$-th relay and the final receiver is then given by $f_{i2}=f_0-f_{i1}$. Because each relay node forwards the signal from the receiver \textit{without decoding}, the forwarded signal still contains the LO frequency offset of the first link. It then follows that all messages arriving at the receiver will carry the same total LO frequency offset of $f_{i1}+f_{i2}=f_0$, which is independent of the relay node $i$. 

\medskip

In practice, things can become more complicated if the LO frequency offsets exhibit significant drift. Suppose the transmitter sends a message at time instant $t_1$. We know that the LO frequency offset satisfies the following condition: 
\begin{equation}
	\label{eq:impl_freq_synch_1}
	f_{i1}(t_1)+f_{i2}(t_1) = f_{j1}(t_1)+f_{j2}(t_1) = f_0(t_1) \ \ \ \ \ \ \ \forall i,j
\end{equation}
However, in reality there is some time delay $T_{d}$ before the relays forward the message to the final receiver. The LO frequency offsets of the different relay nodes will drift independently, such that \eqref{eq:impl_freq_synch_1} is no longer satisfied, which can be expressed by
\begin{equation}
	\label{eq:impl_freq_synch_2}
	f_{i1}(t_1)+f_{i2}(t_1+T_d) \neq f_{j1}(t_1)+f_{j2}(t_1+T_d) \ \ \ \ \ \ \ \forall i,j
\end{equation}
As a result, the signals arriving at the receiver from different relays now have different LO frequency offsets, leading to fading in the total message. 
%In the following subsection, we investigate how the LO drift of our architecture affects the resulting phase error. 



\subsection{Phase error of implicit frequency synchronization}
\label{subsec:phase_error}

We investigate how LO drift affects the properties of implicit frequency synchronization. It will be shown that LO drift causes a zero-mean Gaussian phase error, whose variance can be computed and depends on the system parameters. 

{\bf LO model: }We start by introducing the following LO model: suppose $\phi(t)$ and $\omega(t)$ are the LO phase and (angular) frequency offset at time $t$. The LO phase and frequency offset at time $t+T$ are given by: 
\begin{equation}
	\label{eq:LO_model}
	\left[ \begin{array}{l} \phi(t+T) \\ \omega(t+T) \end{array} \right] = 
							\left[ \begin{array}{l l} 1 & T \\ 0 & 1 \end{array} \right] 
							\left[ \begin{array}{l} \phi(t) \\ \omega(t) \end{array} \right]+ \mathbf{n}(T)
\end{equation}
where $\mathbf{n}(T)$ is the process noise vector, distributed as $\mathbf{n} \sim \mathcal{N}(0,\mathbf{Q}(T))$, which causes the LO phase and frequency offset to drift from their nominal values. In \cite{Zucca:TUFFC:2005,Brown:ICASSP:2012}, it was shown that the process noise covariance matrix $\mathbf{Q}(T)$ can be modeled as 
\begin{equation}
	\label{eq:LO_model_Q}
	\mathbf{Q}\left(T\right) = \omega_c^2 q_1^2 \left[ \begin{array}{c c} T & 0 \\ 0  & 0 \end{array} \right] 
				+ \omega_c^2 q_2^2 \left[ \begin{array}{c c} \frac{T^3}{3} & \frac{T^2}{2} \\	\frac{T^2}{2} & T \end{array} \right]
\end{equation}
where $\omega_c$ is the carrier frequency and the parameters $q_1^2$ and $q_2^2$ are the process noise parameters that correspond to white frequency noise and random walk frequency noise, respectively. 



\medskip

{\bf Intra-cycle drift: } Consider the signal at the final receiver shown in Figure \ref{fig:time_rx_signal}. At time $t_1$, the distant transmitter sends its message to the relays (received with low amplitude), and at time $t_2$, the relays amplify and forward the message to the receiver (received with higher amplitude). The phase of the relayed signal at the receiver is then given by
\begin{align}
	\label{eq:intra_cycle}
	\phi_i(t_2) &= \phi_{i1}(t_1) + \phi_{i2}(t_2) \\
	 						&= \phi_{i1}(t_1) + \phi_{i2}(t_1) + T_d \omega_{i2}(t_1) + n_{\phi_{i2}}(T_d) + \int\limits_{t_1}^{t_2} n_{\omega_{i2}}(\tau) d\tau
\end{align}
where $\phi_{i1}$ and $\phi_{i2}$ denote the phase offset of the long and the short link, $\phi_{i}$ denotes the phase offset of the global link (from transmitter to receiver) through relay $i$, $n_{\phi_{i2}}$ is the LO phase noise over the short link and $n_{\omega_{i2}}$ is the LO frequency noise over the short link. The phase variance due to phase noise is then given by $\omega_c q_1^2 T_d$, whereas the phase increment due to the LO frequency noise is given by $\omega_c q_2^2 \frac{T_d}{3}$ (which follows from the well-known result that for a standard Wiener process $W$, we have that $\int\limits_{a}^{b} W_t dt \sim \mathcal{N}(0,\frac{b-a}{3})$). The total phase error due to intra-cycle drift is thus given by a zero-mean Gaussian process with variance
\begin{equation}
	\label{eq:intra_cycle_var}
	\sigma_{\phi}^2 = \omega_c^2 q_1^2 T_d + \omega_c^2 q_2^2 \frac{T_d^3}{3}
\end{equation}
Intuitively, this can be understood as follows: if the relays wait for a long time before forwarding the message, the LOs of the different relays will drift independently, often resulting in a larger phase error. 
\begin{figure}[ht]
	\centering
	\includegraphics[width=8.5cm]{time_rx_signal}
	\caption{Received signal over two cycles of the setup.}
	\label{fig:time_rx_signal}
\end{figure} 


\medskip

{\bf Inter-cycle drift: } Figure \ref{fig:time_rx_signal} shows several cycles of the setup. At time $t_1$, the transmitter sends a first message, which is forwarded by the relays at time $t_2$. The receiver then computes its feedback message that is returned to the relay nodes; essentially, this message controls the phase $\gamma_i$ that is applied by each relay, such that the total phase $\phi_{i1}(t_1) + \phi_{i2}(t_2) + \gamma_i$ is equal for all links. Now consider a second cycle of the system: at time $t_3$, the transmitter sends another message, which is forwarded by the relays at time $t_4$. The total phase of the second message for link $i$ is given by
\begin{align}
	\label{eq:inter_cycle_1}
	\phi_i(t_2) &= \phi_{i1}(t_3) + \phi_{i2}(t_4) + \gamma_i\\
	\label{eq:inter_cycle_2}
	 						&= \phi_{i1}(t_3) + \phi_{i2}(t_3) + T_d \omega_{i2}(t_3) + n_{\phi_{i2}}(T_d) + \int\limits_{t_3}^{t_4} n_{\omega_{i2}}(\tau) d\tau\ + \gamma_i \\
	\label{eq:inter_cycle_3}
	 						&= \phi_{i1}(t_3) + \phi_{i2}(t_3) + T_d \left( \omega_{i2}(t_1) + n_{\omega_{i2}}(T_c) \right) + n_{\phi_{i2}}(T_d) + \int\limits_{t_3}^{t_4} n_{\omega_{i2}}(\tau) d\tau\ + \gamma_i
\end{align}
where $T_c$ is the cycle time. It can be seen that between $t_1$ and $t_3$ the LO frequency offset $\omega_{i2}$ has drifted, potentially causing the relay phase shift $\gamma_i$ to become outdated. Obviously, if the cycle period gets longer, this drift will be more severe, resulting in a larger phase error. From \eqref{eq:inter_cycle_3}, the total phase error due to both intra- and inter-cycle drift can be characterized by a zero-mean Gaussian process with variance 
\begin{equation}
	\label{eq:inter_cycle_var}
	\sigma_{\phi}^2 = \omega_c^2 q_1^2 T_d + \omega_c^2 q_2^2 \frac{T_d^3}{3} + \omega_c^2 q_2^2 T_d^2 T_c
\end{equation}
The first two terms of the equation are the same as for \eqref{eq:intra_cycle_var} and represent the intra-cycle drift, whereas the last term represent the inter-cycle drift. It can be concluded from \eqref{eq:inter_cycle_var} that, for fixed LO parameters $q_1^2$ and $q_2^2$, both the relay delay time $T_d$ and the cycle time $T_c$ should be kept low to maintain low phase noise. 
 
